Challenges of the Creation of a Dataset for Vision Based Human Hand Action Recognition in Industrial Assembly

This work presents the Industrial Hand Action Dataset V1, an industrial assembly dataset consisting of 12 classes with 459,180 images in the basic version and 2,295,900 images after spatial augmentation. Compared to other freely available datasets tested, it has an above-average duration and, in addition, meets the technical and legal requirements for industrial assembly lines. Furthermore, the dataset contains occlusions, hand-object interaction, and various fine-grained human hand actions for industrial assembly tasks that were not found in combination in examined datasets. The recorded ground truth assembly classes were selected after extensive observation of real-world use cases. A Gated Transformer Network, a state-of-the-art model from the transformer domain was adapted, and proved with a test accuracy of 86.25% before hyperparameter tuning by 18,269,959 trainable parameters, that it is possible to train sequential deep learning models with this dataset.

==> bibliography.tex <==
% ---- Bibliography ----
%
%

@misc{Zhou2018,
  doi = {10.48550/ARXIV.1703.09788},
  
  url = {https://arxiv.org/abs/1703.09788},
  
  author = {Zhou, Luowei and Xu, Chenliang and Corso, Jason J.},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Towards Automatic Learning of Procedures from Web Instructional Videos},
  
  publisher = {arXiv},
  
  year = {2017},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@article{Rohrbach2016,
	doi = {10.1007/s11263-015-0851-8},
  
	url = {https://doi.org/10.1007\%2Fs11263-015-0851-8},
  
	year = 2015,
	month = {8},
  
	publisher = {Springer Science and Business Media {LLC}
},
  
	volume = {119},
  
	number = {3},
  
	pages = {346--373},
  
	author = {Marcus Rohrbach and Anna Rohrbach and Michaela Regneri and Sikandar Amin and\linebreak Mykhaylo Andriluka and Manfred Pinkal and Bernt Schiele},
  
	title = {Recognizing Fine-Grained and Composite Activities Using Hand-Centric Features and Script Data},
  
	journal = {International Journal of Computer Vision}
}

@misc{egtea,
  doi = {10.48550/ARXIV.2006.00626},
  
  url = {https://arxiv.org/abs/2006.00626},
  
  author = {Li, Yin and Liu, Miao and Rehg, James M.},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {In the Eye of the Beholder: Gaze and Actions in First Person Video},
  
  publisher = {arXiv},
  
  year = {2020},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@INPROCEEDINGS{EgoHands,  author={Bambach, Sven and Lee, Stefan and Crandall, David J. and Yu, Chen},  booktitle={2015 IEEE International Conference on Computer Vision (ICCV)},   title={Lending A Hand: Detecting Hands and Recognizing Activities in Complex Egocentric Interactions},   year={2015},  volume={},  number={},  pages={1949-1957},  doi={10.1109/ICCV.2015.226}}

@article{Tang2019,
  author    = {Yansong Tang and
               Dajun Ding and
               Yongming Rao and
               Yu Zheng and
               Danyang Zhang and
               Lili Zhao and
               Jiwen Lu and
               Jie Zhou},
  title     = {{COIN:} {A} Large-scale Dataset for Comprehensive Instructional Video
               Analysis},
  journal   = {CoRR},
  volume    = {abs/1903.02874},
  year      = {2019},
  url       = {http://arxiv.org/abs/1903.02874},
  eprinttype = {arXiv},
  eprint    = {1903.02874},
  timestamp = {Thu, 23 May 2019 17:54:35 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1903-02874.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@INPROCEEDINGS{tensorcanonical,  author={Kim, Tae-Kyun and Wong, Shu-Fai and Cipolla, Roberto},  booktitle={2007 IEEE Conference on Computer Vision and Pattern Recognition},   title={Tensor Canonical Correlation Analysis for Action Classification},   year={2007},  volume={},  number={},  pages={1-8},  doi={10.1109/CVPR.2007.383137}}

@ARTICLE{Zhang2018,  author={Zhang, Yifan and Cao, Congqi and Cheng, Jian and Lu, Hanqing},  journal={IEEE Transactions on Multimedia},   title={EgoGesture: A New Dataset and Benchmark for Egocentric Hand Gesture Recognition},   year={2018},  volume={20},  number={5},  pages={1038-1050},  doi={10.1109/TMM.2018.2808769}}

@article{Zhang2020,
  author    = {Fan Zhang and
               Valentin Bazarevsky and
               Andrey Vakunov and
               Andrei Tkachenka and
               George Sung and
               Chuo{-}Ling Chang and
               Matthias Grundmann},
  title     = {MediaPipe Hands: On-device Real-time Hand Tracking},
  journal   = {CoRR},
  volume    = {abs/2006.10214},
  year      = {2020},
  url       = {https://arxiv.org/abs/2006.10214},
  eprinttype = {arXiv},
  eprint    = {2006.10214},
  timestamp = {Tue, 23 Jun 2020 17:57:22 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2006-10214.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-2005-02134,
  author    = {Gibran Benitez{-}Garcia and
               Jesus Olivares{-}Mercado and
               Gabriel Sanchez{-}Perez and
               Keiji Yanai},
  title     = {{IPN} Hand: {A} Video Dataset and Benchmark for Real-Time Continuous
               Hand Gesture Recognition},
  journal   = {CoRR},
  volume    = {abs/2005.02134},
  year      = {2020},
  url       = {https://arxiv.org/abs/2005.02134},
  eprinttype = {arXiv},
  eprint    = {2005.02134},
  timestamp = {Fri, 08 May 2020 15:04:04 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2005-02134.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{multi-modal_hands,
place = {Country unknown/Code not available}, title = {First-Person View Hand Segmentation of Multi-Modal Hand Activity Video Dataset.}, url = {https://par.nsf.gov/biblio/10297591}, abstractNote = {First-person-view videos of hands interacting with tools are widely used in the computer vision industry. However, creating a dataset with pixel-wise segmentation of hands is challenging since most videos are captured with fingertips occluded by the hand dorsum and grasped tools. Current methods often rely on manually segmenting hands to create annotations, which is inefficient and costly. To relieve this challenge, we create a method that utilizes thermal information of hands for efficient pixel-wise hand segmentation to create a multi-modal activity video dataset. Our method is not affected by fingertip and joint occlusions and does not require hand pose ground truth. We show our method to be 24 times faster than the traditional polygon labeling method while maintaining high quality. With the segmentation method, we propose a multi-modal hand activity video dataset with 790 sequences and 401,765 frames of "hands using tools" videos captured by thermal and RGB-D cameras with hand segmentation data. We analyze multiple models for hand segmentation performance and benchmark four segmentation networks. We show that our multi-modal dataset with fusing Long-Wave InfraRed (LWIR) and RGB-D frames achieves 5\% better hand IoU performance than using RGB frames.}, journal = {BMVC 2020}, author = {Sangpil Kim, Hyung-Gun Chi},year={2020} }


@inproceedings{workinghands,
  title={WorkingHands: A Hand-Tool Assembly Dataset for Image Segmentation and Activity Mining},
  author={Roy Shilkrot and Supreeth Narasimhaswamy and Saif Vazir and Minh Hoai},
  booktitle={BMVC},
  year={2019}
}

@article{IKEAASM,
  author    = {Yizhak Ben{-}Shabat and
               Xin Yu and
               Fatemeh Sadat Saleh and
               Dylan Campbell and
               Cristian Rodriguez Opazo and
               Hongdong Li and
               Stephen Gould},
  title     = {The {IKEA} {ASM} Dataset: Understanding People Assembling Furniture
               through Actions, Objects and Pose},
  journal   = {CoRR},
  volume    = {abs/2007.00394},
  year      = {2020},
  url       = {https://arxiv.org/abs/2007.00394},
  eprinttype = {arXiv},
  eprint    = {2007.00394},
  timestamp = {Thu, 14 Oct 2021 09:14:54 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2007-00394.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-2201-05761,
  author    = {Alexandre Lopes and
               Roberto Souza and
               H{\'{e}}lio Pedrini},
  title     = {A Survey on {RGB-D} Datasets},
  journal   = {CoRR},
  volume    = {abs/2201.05761},
  year      = {2022},
  url       = {https://arxiv.org/abs/2201.05761},
  eprinttype = {arXiv},
  eprint    = {2201.05761},
  timestamp = {Thu, 08 Sep 2022 21:08:20 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2201-05761.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inbook{BDSG,
author = {},
editor = {Kai-Uwe Plath},
doi = {doi:10.9785/ovs.9783504380403.xv},
url = {https://doi.org/10.9785/ovs.9783504380403.xv},
title = {Bundesdatenschutzgesetz (BDSG): in der Fassung der Bekanntmachung vom 14. Januar 2003 (BGBl. I S. 66), zuletzt geändert durch Gesetz vom 14. August 2009 (BGBl. I S. 2814)},
booktitle = {BDSG: Kommentar zum BDSG sowie den Datenschutzbestimmungen des TMG und TKG},
year = {2012},
publisher = {Verlag Dr. Otto Schmidt},
pages = {XV--LXI},
lastchecked = {2022-05-10}
}

@article{Jauch2021,
author = {Jauch, Christian and Denecke, Julia and Huber, Marco},
year = {2021},
month = {01},
pages = {119-1},
title = {Generating a Hand Pose Data Set for Vision Based Manual Assembly Assistance Systems},
volume = {2021},
journal = {Electronic Imaging},
doi = {10.2352/ISSN.2470-1173.2021.18.3DIA-119}
}

@INPROCEEDINGS{lttm1,  author={Marin, Giulio and Dominio, Fabio and Zanuttigh, Pietro},  booktitle={2014 IEEE International Conference on Image Processing (ICIP)},   title={Hand gesture recognition with leap motion and kinect devices},   year={2014},  volume={},  number={},  pages={1565-1569},  doi={10.1109/ICIP.2014.7025313}}

@Article{lttm2,
author={Marin, Giulio
and Dominio, Fabio
and Zanuttigh, Pietro},
title={Hand gesture recognition with jointly calibrated Leap Motion and depth sensor},
journal={Multimedia Tools and Applications},
year={2016},
month={11},
day={01},
volume={75},
number={22},
pages={14991-15015},
abstract={Novel 3D acquisition devices like depth cameras and the Leap Motion have recently reached the market. Depth cameras allow to obtain a complete 3D description of the framed scene while the Leap Motion sensor is a device explicitly targeted for hand gesture recognition and provides only a limited set of relevant points. This paper shows how to jointly exploit the two types of sensors for accurate gesture recognition. An ad-hoc solution for the joint calibration of the two devices is firstly presented. Then a set of novel feature descriptors is introduced both for the Leap Motion and for depth data. Various schemes based on the distances of the hand samples from the centroid, on the curvature of the hand contour and on the convex hull of the hand shape are employed and the use of Leap Motion data to aid feature extraction is also considered. The proposed feature sets are fed to two different classifiers, one based on multi-class SVMs and one exploiting Random Forests. Different feature selection algorithms have also been tested in order to reduce the complexity of the approach. Experimental results show that a very high accuracy can be obtained from the proposed method. The current implementation is also able to run in real-time.},
issn={1573-7721},
doi={10.1007/s11042-015-2451-6},
url={https://doi.org/10.1007/s11042-015-2451-6}
}



@Article{chalearn,
author={Guyon, Isabelle
and Athitsos, Vassilis
and Jangyodsuk, Pat
and Escalante, Hugo Jair},
title={The ChaLearn gesture dataset (CGD 2011)},
journal={Machine Vision and Applications},
year={2014},
month={11},
day={01},
volume={25},
number={8},
pages={1929-1951},
abstract={This paper describes the data used in the ChaLearn gesture challenges that took place in 2011/2012, whose results were discussed at the CVPR 2012 and ICPR 2012 conferences. The task can be described as: user-dependent, small vocabulary, fixed camera, one-shot-learning. The data include 54,000 hand and arm gestures recorded with an RGB-D {\$}{\$}{\backslash}hbox {\{}Kinect{\}}^{\backslash}mathrm{\{}TM{\}}{\$}{\$}camera. The data are organized into batches of 100 gestures pertaining to a small gesture vocabulary of 8--12 gestures, recorded by the same user. Short continuous sequences of 1--5 randomly selected gestures are recorded. We provide man-made annotations (temporal segmentation into individual gestures, alignment of RGB and depth images, and body part location) and a library of function to preprocess and automatically annotate data. We also provide a subset of batches in which the user's horizontal position is randomly shifted or scaled. We report on the results of the challenge and distribute sample code to facilitate developing new solutions. The data, datacollection software and the gesture vocabularies are downloadable from http://gesture.chalearn.org. We set up a forum for researchers working on these data http://groups.google.com/group/gesturechallenge.},
issn={1432-1769},
doi={10.1007/s00138-014-0596-3},
url={https://doi.org/10.1007/s00138-014-0596-3}
}

@article{Liu2021,
  author    = {Minghao Liu and
               Shengqi Ren and
               Siyuan Ma and
               Jiahui Jiao and
               Yizhou Chen and
               Zhiguang Wang and
               Wei Song},
  title     = {Gated Transformer Networks for Multivariate Time Series Classification},
  journal   = {CoRR},
  volume    = {abs/2103.14438},
  year      = {2021},
  url       = {https://arxiv.org/abs/2103.14438},
  eprinttype = {arXiv},
  eprint    = {2103.14438},
  timestamp = {Wed, 07 Apr 2021 15:31:46 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2103-14438.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Carreira2017,
  author    = {Jo{\~{a}}o Carreira and
               Andrew Zisserman},
  title     = {Quo Vadis, Action Recognition? {A} New Model and the Kinetics Dataset},
  journal   = {CoRR},
  volume    = {abs/1705.07750},
  year      = {2017},
  url       = {http://arxiv.org/abs/1705.07750},
  eprinttype = {arXiv},
  eprint    = {1705.07750},
  timestamp = {Mon, 13 Aug 2018 16:47:23 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/CarreiraZ17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@InProceedings{driveandact,
author = {Martin, Manuel and Roitberg, Alina and Haurilet, Monica and Horne, Matthias and Reiß, Simon and Voit, Michael and Stiefelhagen, Rainer},
title = {Drive\&Act: A Multi-modal Dataset for Fine-grained Driver Behavior Recognition in Autonomous Vehicles},
booktitle = {The IEEE International Conference on Computer Vision (ICCV)},
month = {10},
year = {2019}
}

@INPROCEEDINGS{rogez,  author={Rogez, Grégory and Supancic, James S. and Ramanan, Deva},  booktitle={2015 IEEE International Conference on Computer Vision (ICCV)},   title={Understanding Everyday Hands in Action from RGB-D Images},   year={2015},  volume={},  number={},  pages={3889-3897},  doi={10.1109/ICCV.2015.443}}

@article{Goyal2017,
  author    = {Raghav Goyal and
               Samira Ebrahimi Kahou and
               Vincent Michalski and
               Joanna Materzynska and
               Susanne Westphal and
               Heuna Kim and
               Valentin Haenel and
               Ingo Fr{\"{u}}nd and
               Peter Yianilos and
               Moritz Mueller{-}Freitag and
               Florian Hoppe and
               Christian Thurau and
               Ingo Bax and
               Roland Memisevic},
  title     = {The "something something" video database for learning and evaluating
               visual common sense},
  journal   = {CoRR},
  volume    = {abs/1706.04261},
  year      = {2017},
  url       = {http://arxiv.org/abs/1706.04261},
  eprinttype = {arXiv},
  eprint    = {1706.04261},
  timestamp = {Mon, 13 Aug 2018 16:48:38 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/GoyalKMMWKHFYMH17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{aisha,
  author    = {Aisha Urooj Khan and
               Ali Borji},
  title     = {Analysis of Hand Segmentation in the Wild},
  journal   = {CoRR},
  volume    = {abs/1803.03317},
  year      = {2018},
  url       = {http://arxiv.org/abs/1803.03317},
  eprinttype = {arXiv},
  eprint    = {1803.03317},
  timestamp = {Mon, 13 Aug 2018 16:47:13 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1803-03317.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@ARTICLE{Ji2013,  author={Ji, Shuiwang and Xu, Wei and Yang, Ming and Yu, Kai},  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},   title={3D Convolutional Neural Networks for Human Action Recognition},   year={2013},  volume={35},  number={1},  pages={221-231},  doi={10.1109/TPAMI.2012.59}}

@article{Feichtenhofer2016,
  author    = {Christoph Feichtenhofer and
               Axel Pinz and
               Andrew Zisserman},
  title     = {Convolutional Two-Stream Network Fusion for Video Action Recognition},
  journal   = {CoRR},
  volume    = {abs/1604.06573},
  year      = {2016},
  url       = {http://arxiv.org/abs/1604.06573},
  eprinttype = {arXiv},
  eprint    = {1604.06573},
  timestamp = {Mon, 13 Aug 2018 16:45:57 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/FeichtenhoferPZ16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@INPROCEEDINGS{Singh2016,  author={Singh, Bharat and Marks, Tim K. and Jones, Michael and Tuzel, Oncel and Shao, Ming},  booktitle={2016 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},   title={A Multi-stream Bi-directional Recurrent Neural Network for Fine-Grained Action Detection},   year={2016},  volume={},  number={},  pages={1961-1970},  doi={10.1109/CVPR.2016.216}}

==> reminder <==
\begin{thebibliography}{6}
%
\bibitem{Zhou2018}Zhou, L., Xu, C. \& Corso, J. ProcNets: Learning to Segment Procedures in Untrimmed and Unconstrained Videos. {\em CoRR}. \textbf{abs/1703.09788} (2017), http://arxiv.org/abs/1703.09788

\bibitem{Rohrbach2016}Rohrbach, M., Rohrbach, A., Regneri, M., Amin, S., Andriluka, M., Pinkal, M. \& Schiele, B. Recognizing Fine-Grained and Composite Activities Using Hand-Centric Features and Script Data. {\em International Journal Of Computer Vision}. \textbf{119}, 346-373 (2016,9)

\bibitem{egtea}Li, Y., Liu, M. \& Rehg, J. In the Eye of the Beholder: Gaze and Actions in First Person Video. {\em CoRR}. \textbf{abs/2006.00626} (2020), https://arxiv.org/abs/2006.00626

\bibitem{EgoHands}Bambach, S., Lee, S., Crandall, D., Psychological, C. \& Sciences, B. Lending A Hand: Detecting Hands and Recognizing Activities in Complex Egocentric Interactions.  (2015), http://vision.soic.indiana.edu/egohands/

\bibitem{Tang2019}Tang, Y., Ding, D., Rao, Y., Zheng, Y., Zhang, D., Zhao, L., Lu, J. \& Zhou, J. COIN: A Large-scale Dataset for Comprehensive Instructional Video Analysis. {\em CoRR}. \textbf{abs/1903.02874} (2019), http://arxiv.org/abs/1903.02874

\bibitem{tensorcanonical}Kim, T., Wong, S. \& Cipolla, R. Tensor Canonical Correlation Analysis for Action Classification. {\em 2007 IEEE Conference On Computer Vision And Pattern Recognition}. pp. 1-8 (2007)

\bibitem{Zhang2018}Zhang, Y., Cao, C., Cheng, J. \& Lu, H. EgoGesture: A New Dataset and Benchmark for Egocentric Hand Gesture Recognition. {\em IEEE Transactions On Multimedia}. \textbf{20}, 1038-1050 (2018,5)

\bibitem{Zhang2020}Zhang, F., Bazarevsky, V., Vakunov, A., Tkachenka, A., Sung, G., Chang, C. \& Grundmann, M. MediaPipe Hands: On-device Real-time Hand Tracking. {\em CoRR}. \textbf{abs/2006.10214} (2020), https://arxiv.org/abs/2006.10214

\bibitem{DBLP:journals/corr/abs-2005-02134}Benitez-Garcia, G., Olivares-Mercado, J., Sanchez-Perez, G. \& Yanai, K. IPN Hand: A Video Dataset and Benchmark for Real-Time Continuous Hand Gesture Recognition. {\em CoRR}. \textbf{abs/2005.02134} (2020), https://arxiv.org/abs/2005.02134

\bibitem{multi-modal_hands}Kim, S., Hu, X., Vegesana, A. \& Ramani, K. First-Person View Hand Segmentation of Multi-Modal Hand Activity Video Dataset. {\em BMVC}. (2020)

\bibitem{workinghands}Shilkrot, R., Narasimhaswamy, S., Vazir, S. \& Hoai, M. WorkingHands: A Hand-Tool Assembly Dataset for Image Segmentation and Activity Mining.  (2019), http://hi.cs.stonybrook.edu/workinghands.

\bibitem{IKEAASM}Ben-Shabat, Y., Yu, X., Saleh, F., Campbell, D., Opazo, C., Li, H. \& Gould, S. The IKEA ASM Dataset: Understanding People Assembling Furniture through Actions, Objects and Pose. {\em CoRR}. \textbf{abs/2007.00394} (2020), https://arxiv.org/abs/2007.00394

\bibitem{DBLP:journals/corr/abs-2201-05761}Lopes, A., Souza, R. \& Pedrini, H. A Survey on RGB-D Datasets. {\em CoRR}. \textbf{abs/2201.05761} (2022), https://arxiv.org/abs/2201.05761

\bibitem{BDSG}European Union, C. Bundesdatenschutzgesetz (BDSG): in der Fassung der Bekanntmachung vom 14. Januar 2003 (BGBl. I S. 66), zuletzt geändert durch Gesetz vom 14. August 2009 (BGBl. I S. 2814). {\em BDSG: Kommentar Zum BDSG Sowie Den Datenschutzbestimmungen Des TMG Und TKG}. pp. XV-LXI (2012), https://doi.org/10.9785/ovs.9783504380403.xv

%@inbook{BDSG,
%author = {},
%editor = {Kai-Uwe Plath},
%doi = {doi:10.9785/ovs.9783504380403.xv},
%url = {https://doi.org/10.9785/ovs.9783504380403.xv},
%title = {Bundesdatenschutzgesetz (BDSG): in der Fassung der Bekanntmachung vom 14. Januar 2003 (BGBl. I S. 66), zuletzt geändert durch Gesetz vom 14. August 2009 (BGBl. I S. 2814)},
%booktitle = {BDSG: Kommentar zum BDSG sowie den Datenschutzbestimmungen des TMG und TKG},
%year = {2012},
%publisher = {Verlag Dr. Otto Schmidt},
%pages = {XV--LXI},
%lastchecked = {2022-05-10}
%}

\bibitem{Jauch2021}Jauch, C., Denecke, J. \& Huber, M. Generating a Hand Pose Data Set for Vision Based Manual Assembly Assistance Systems. {\em Electronic Imaging}. \textbf{2021}, 119-1-119-7 (2021,2)

\bibitem{lttm1}Marin, G., Dominio, F. \& Zanuttigh, P. Hand gesture recognition with leap motion and kinect devices. {\em 2014 IEEE International Conference On Image Processing (ICIP)}. pp. 1565-1569 (2014)

\bibitem{lttm2}Marin, G., Dominio, F. \& Zanuttigh, P. Hand gesture recognition with jointly calibrated Leap Motion and depth sensor. {\em Multimedia Tools And Applications}. \textbf{75}, 14991-15015 (2016,11)

\bibitem{chalearn}Guyon, I., Athitsos, V., Jangyodsuk, P., Hugo, ·., Escalante, J., Jair, H. \& Inaoe, E. The ChaLearn Gesture Dataset (CGD 2011).  (2011), http://groups.google.com/group/gesturechallenge.

\bibitem{Liu2021}Liu, M., Ren, S., Ma, S., Jiao, J., Chen, Y., Wang, Z. \& Song, W. Gated Transformer Networks for Multivariate Time Series Classification. {\em CoRR}. \textbf{abs/2103.14438} (2021), https://arxiv.org/abs/2103.14438

\bibitem{Carreira2017}Carreira, J. \& Zisserman, A. Quo Vadis, Action Recognition? A New Model and the Kinetics Dataset. {\em CoRR}. \textbf{abs/1705.07750} (2017), http://arxiv.org/abs/1705.07750

\bibitem{driveandact}Martin, M., Roitberg, A., Haurilet, M., Horne, M., Reiß, S., Voit, M. \& Stiefelhagen, R. Drive\&Act: A Multi-modal Dataset for Fine-grained Driver Behavior Recognition in Autonomous Vehicles.  (2019), www.driveandact.com

\bibitem{rogez}Rogez, G., Supancic, J. \& Ramanan, D. Understanding Everyday Hands in Action from RGB-D Images. {\em 2015 IEEE International Conference On Computer Vision (ICCV)}. pp. 3889-3897 (2015)

\bibitem{Goyal2017}Goyal, R., Kahou, S., Michalski, V., Materzynska, J., Westphal, S., Kim, H., Haenel, V., Fründ, I., Yianilos, P., Mueller-Freitag, M., Hoppe, F., Thurau, C., Bax, I. \& Memisevic, R. The "something something" video database for learning and evaluating visual common sense. {\em CoRR}. \textbf{abs/1706.04261} (2017), http://arxiv.org/abs/1706.04261

\bibitem{aisha}Khan, A. \& Borji, A. Analysis of Hand Segmentation in the Wild. {\em CoRR}. \textbf{abs/1803.03317} (2018), http://arxiv.org/abs/1803.03317

\bibitem{Ji2013}Ji, S., Xu, W., Yang, M. \& Yu, K. 3D Convolutional neural networks for human action recognition. {\em IEEE Transactions On Pattern Analysis And Machine Intelligence}. \textbf{35}, 221-231 (2013)

\bibitem{Feichtenhofer2016}Feichtenhofer, C., Pinz, A. \& Zisserman, A. Convolutional Two-Stream Network Fusion for Video Action Recognition. {\em CoRR}. \textbf{abs/1604.06573} (2016), http://arxiv.org/abs/1604.06573

\bibitem{Singh2016}Singh, B., Marks, T., Jones, M., Tuzel, C., Oncel, ;., Shao, M., Singh, B., Marks, T., Jones, M. \& Tuzel, O. A Multi-Stream Bi-Directional Recurrent Neural Network for Fine-Grained Action Detection.  (2016), http://www.merl.com
\end{thebibliography}
